Learning Parametrised Graph Shift Operators

In many domains data is currently represented as graphs and therefore, the graph representation of this data becomes increasingly important in machine learning. Network data is, implicitly or explicitly, always represented using a graph shift operator (GSO) with the most common choices being the adjacency, Laplacian matrices and their normalisations. In this paper, a novel parametrised GSO (PGSO) is proposed, where specific parameter values result in the most commonly used GSOs and message-passing operators in graph neural network (GNN) frameworks. The PGSO is suggested as a replacement of the standard GSOs that are used in state-of-the-art GNN architectures and the optimisation of the PGSO parameters is seamlessly included in the model training. It is proved that the PGSO has real eigenvalues and a set of real eigenvectors independent of the parameter values and spectral bounds on the PGSO are derived. PGSO parameters are shown to adapt to the sparsity of the graph structure in a study on stochastic blockmodel networks, where they are found to automatically replicate the GSO regularisation found in the literature. On several real-world datasets the accuracy of state-of-the-art GNN architectures is improved by the inclusion of the PGSO in both node- and graph-classification tasks.

==> chapters/genlap_empirical.tex <==
\section{Interpretability of the generalised Laplacian parameters -- Empirical results} \label{sec:genlap_empirical}
In this section, we provide empirical insights on the behavior of the parameter set of  \genlapout with respect to different user-end tasks.

It would be nice to start this section with our defintion of interpretability, so that we are not arguing with reviewers whether our operator is interpretable. But rather whether our definition of interpretability is realistic.


\subsection{Stochastic block models and sparsity levels }

On this section, we investigate on the behavior of the \genlapout parameters with respect to the sparsity level of the graph. Towards this, we evaluate the expressivity of the \genlapout representation on graphs generated by \textbf{stochastic blockmodels}.
\subsubsection{Stochastic Blockmodel}
\begin{itemize}
    \item Description, parameters
    \item Usage, applications
\end{itemize}

\paragraph{Experiment Setup}{We generate 20 graphs using a varying set of probabilities $p,q$. We vary $p,q$ so that we keep in constant the ratio $\frac{p}{q}$ while moving on different sparsity levels. Keeping the ratio $\frac{p}{q}$ in constant allows us to retain the detectability of the communities inside the graph. In particular, as Figureo \ref{fig:graphs_sbm} shows the ordered adjacency matrix of each graph contain highly detectable communities. Each graph contains a fixed number of nodes equal to 300 and each node has a label that corresponds to its community membership and an uninformatice node attribute vector. We evaluate the performance of the models using \genlapout on a classical node classification task with 3 classes.}

\begin{figure}[h!]
\begin{subfigure}{0.5\textwidth}
\centering
    \includegraphics[scale=0.4]{figures/genlap_parameters_sparsity_levels_15_init0.pdf}
    \caption{Behavior of \genlapout parameters for different sparsity levels of SBM. Naive weight initialization.}
    \label{fig:sbm_init0}

\end{subfigure}
 \begin{subfigure}{0.5\textwidth}
\centering
    \includegraphics[scale=0.4]{figures/genlap_parameters_sparsity_levels_15_initGCN.pdf}
    \caption{Behavior of \genlapout parameters for different sparsity levels of SBM. Default GCN initialization.}
    \label{fig:sbm_initGCN}

\end{subfigure}
    
\end{figure}

\subsection{Behavior of multiplicative parameters $c_1, c_2, c_3$}

Looking back at Equation \eqnref{eq:genlap}, we can classify the roles of the parameters with regards to their application on either the degree matrix $D$ or the adjacency matrix $A$. The term $c_2 D_{\addparain}^qA_{\addparain} D_{\addparain}^r$ represents the information that we gather from the direct neighborhood, while the terms  $c_3 D^p$ and  $c_1 I_n$ have an impact on the nodewise self-importance in comparison with the neighborhood importance. This observation drives into an assumption that for different problem setups, the \genlapout parameters  should play different roles.
\paragraph{Graph Classification:} In the literature, the standard graph classification benchmarks contain small in size and sparse graphs. Usually, the learned graph-level representations aggregate the node-level representations in an effort to capture the most structural and contextual information from the graph itself. Intuitively, we expect weights that correspond to the interactions between a nodes and its neighbors to play a significant role.
\paragraph{Node Classification:} On the other hand, the node classification benchmarks consist of larger in size and usually denser denser graphs, where the node-level embeddings play a significant role of expressing the nodewise information. In contrast to the graph classification setup, we expect the weights that represent the self-importance of a node to have a higher impact. \\\\
The application of \genlapout allows us to facilitate this comparison by examining three standard node classification and two graph classification datasets, as it is shown in Figure \ref{fig:c2_nc_vs_gc}.

\begin{figure}[h!]
    \begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[scale=0.16]{node_classification_c2.png}
    \caption{Node Classification}
    \label{fig:c2_node_classification}
    \end{subfigure}
    \begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[scale=0.16]{graph_classification_c2.png}
    \caption{Graph Classification}
    \label{fig:c2_graph_classification}
    \end{subfigure}
    \caption{Behavior of $c_2$ parameter in two user-end tasks}
    \label{fig:c2_nc_vs_gc}
\end{figure}

On Figure \ref{fig:c2_node_classification}, we can observe that $c_2$ parameter, which corresponds to the adjacency matrix term of  \genlapout takes negative values around zero (the exception is the case of PubMed, where it seems that it diverges), while on Figure \ref{fig:c2_graph_classification}, we observe a mirroring trend, where $c_2$ parameters takes positive values. This indicates a possible opposite correlation of the neighborhood importance with respect to the two different taks. 


\subsection{Stochastic block models and sparsity levels }






==> chapters/potentially_add_if_time.tex <==
Discuss that the GAT consists of several attention-update steps which are run in parallel and then aggregated. The GIN runs message passing update layers sequentially and then aggregated the hidden states. The GCN simply runs message passsing update layers in sequence. 

Add SBM convergence speed improvement

monitor the condition number and Gershgorin intervals over all graphs in the dataset for graph classification

Since we change the representation of a whole graph at a time it could have been expected that this approach offers a greater improvement on graph classification rather than on node classification.

Early on in the project we drew the conclusion that we are doing better in datasets without many node features. We explained this by us improving the representation of neighbourhoods and therefore only the representation of topological and not feature data. Does this still apply to the new results?




PROBABLY WRONG:
We consistently find (m_1, m_3) and m_2 to have opposing sign. Hence, the signless Laplacian never seems to optimally reprensent our datasets.

THIS IS IGNORING THE LINEAR TRANSFORMATION IN THE UPDATE STEP... We observed positive (m_1, m_3) and negative m_2 for node-classification tasks and vice versa for graph classification. Since the GNNs we train have RELU activation functions a negative multiplicative parameter can be seen as an attempt to filter this part of the signal. Therefore, we interpreted this phenomenon as the individual node signal having greater importance than the signal arising at neighbours in the node classification task, while in graph classification the signal of neighbours has a larger contribution towards achieving the task.






==> chapters/preliminaries.tex <==
\section{Preliminaries}
We define a graph $G$ as a tuple $G=(V,E)$, where $V,E$ are the sets of nodes and edges respectively ($|V| = n, |M|=m$) and $U \in \mathbb{R}^{n\times n\times d}$ is the attribute tensor, where the diagonal entries $u_{ii\cdot}$ denote the node attribute vectors and the off-diagonal entries $u_{ij\cdot}$ denote the edge attributes ($u_{ij}=0$ if there is no edge between $i,j$). 
(For example, in GCNs with node attributes they are using the X = diag(U), where $\text{diag_{ii\cdot}}$ extracts the diagonal elements of our tensor with the first two dimensions being fixed.)


\subsection{Graph-shift operators and filters on graphs}
Although the terms of the adjacency matrix and laplacian operator seem to be defined with the foundations of the graph theory, the notions of graph shifting and graph shift operators have  been defined very recently \citep{Sandryhaila2013, Shuman2013}. 
\begin{definition}{\textbf{Graph Shift Operator}} A matrix $S \in \mathbb{R}^{n \times n}$ is called a \textit{Graph-Shift Operator} (GSO) if it satisfies $S_{i,j}=0 \text{ for } i \neq j \text{ and } (i,j) \notin E$. \textbf{consider adding the fact that it should be non-zero when edges are present}
\end{definition}
It is clear that both the adjacency matrix and unnormalized/normalized variants of the Laplacian operator fall under Definition 1.

\begin{definition} {\textbf{Graph Filter}}

\end{definition}
